PrivTree: A Differentially Private Algorithm for Hierarchical Decompositions

Given a set D of tuples defined on a domain Omega, we study differentially private algorithms for constructing a histogram over Omega to approximate the tuple distribution in D. Existing solutions for the problem mostly adopt a hierarchical decomposition approach, which recursively splits Omega into sub-domains and computes a noisy tuple count for each sub-domain, until all noisy counts are below a certain threshold. This approach, however, requires that we (i) impose a limit h on the recursion depth in the splitting of Omega and (ii) set the noise in each count to be proportional to h. This leads to inferior data utility due to the following dilemma: if we use a small h, then the resulting histogram would be too coarse-grained to provide an accurate approximation of data distribution; meanwhile, a large h would yield a fine-grained histogram, but its quality would be severely degraded by the increased amount of noise in the tuple counts. To remedy the deficiency of existing solutions, we present PrivTree, a histogram construction algorithm that also applies hierarchical decomposition but features a crucial (and somewhat surprising) improvement: when deciding whether or not to split a sub-domain, the amount of noise required in the corresponding tuple count is independent of the recursive depth. This enables PrivTree to adaptively generate high-quality histograms without even asking for a pre-defined threshold on the depth of sub-domain splitting. As concrete examples, we demonstrate an application of PrivTree in modelling spatial data, and show that it can also be extended to handle sequence data (where the decision in sub-domain splitting is not based on tuple counts but a more sophisticated measure). Our experiments on a variety of real datasets show that PrivTree significantly outperforms the states of the art in terms of data utility.

==> 2-Preliminaries/Preliminaries2.tex <==
\section{Preliminaries}\label{sec:pre}
%This section reviews two concepts closely related to our work, namely, differential privacy and spatial decomposition.

In this section, we introduce the concepts behind {\em differential privacy} \cite{D06}, and formally define the problem of {\em spatial decomposition} \cite{}, which we will address with our {\em PrivTree} algorithm in Section~\ref{sec:alg}. 

\subsection{Differential Privacy}\label{sec:pre-dp}

%We now introduce the concepts behind differential privacy\cite{DMNS06}. Let $D$ be a sensitive dataset of $n$ tuples, and $f$ be the query of interest. Differential privacy
%requires that the release of $f(D)$ should not reveal much information about any particular tuple in $D$. Intuitively, this implies that the impact of any single tuple to the output would be little.
%The formal definition of differential privacy is as follows:
%\begin{definition}[$\e$-Differential Privacy] \label{def:pre-dp}
%A randomized algorithm $\mathcal{A}$ satisfies $\e$-differential
%privacy, if for any two datasets $D$ and $D'$ that differ only in one tuple, and for any possible output $O$ of $\mathcal{A}$, we have
%\begin{equation} \label{eqn:prelim-epsilon}
%\Pr\left[\mathcal{A}(D) = O \right] \le e^{\varepsilon} \cdot \Pr\left[\mathcal{A}(D') = O\right],
%\end{equation}
%where $\Pr[\cdot]$ denotes the probability of an event.
%\end{definition}
%In what follows, we say that two datasets are {\it neighboring} if they differ in only one tuple, i.e., the tuple is present in only one of the two datasets while the rest are identical.
%Although there are many approaches to achieving differential privacy,
%the most fundamental one is the {\em Laplace mechanism}~\cite{DMNS06}.


%we describe the two best known and most-widely used,
%namely, the {\em Laplace mechanism} \cite{DMNS06} and the
%{\em exponential mechanism} \cite{MT07}.

Let $D$ be a sensitive dataset with $n$ tuples, and $\mathcal{A}$ be a data publishing algorithm that takes $D$ as input and releases a set of information $\mathcal{A}(D)$. Differential privacy requires that $\mathcal{A}(D)$ should be insensitive to the presence or absence of any particular tuple in $D$, so that an adversary cannot infer much private information from $\mathcal{A}(D)$. More formally, differential privacy is defined based on the concept of {\em neighboring datasets}, as shown in the following. 

\begin{definition}[Neighboring Datasets \cite{D06}] \label{def:pre-neighbor}
Two datasets are neighboring if one of them can be obtained by inserting a tuple into the other.
\end{definition}

\begin{definition}[$\e$-Differential Privacy \cite{D06}] \label{def:pre-dp}
A randomized algorithm $\mathcal{A}$ satisfies $\e$-differential privacy if, for any two neighboring datasets $D$ and $D'$ and for any possible output $O$ of $\mathcal{A}$, we have
\begin{equation} \label{eqn:pre-epsilon}
\Pr\left[\mathcal{A}(D) = O \right] \le e^{\varepsilon} \cdot \Pr\left[\mathcal{A}(D') = O\right],
\end{equation}
where $\Pr[\cdot]$ denotes the probability of an event.
\end{definition}

There exist several mechanisms \cite{} for achieving differential privacy, among which the most fundamental one is the {\em Laplace mechanism}. Specifically, the Laplace mechanism considers a function $f$ that takes $D$ as input and outputs a vector of real numbers, and it aims to release $f(D)$ with differential privacy. To achieve this objective, it adds i.i.d.\ noise into each value in $f(D)$, such that the noise $\eta$ follows a {\em Laplace distribution} with the following probability density function:
\begin{equation} \label{eqn:pre-laplace}
\Pr[\eta = x] = \frac{1}{2\lambda} e^{-|x|/\lambda}.
\end{equation}
We denote the above distribution as $\Lap(\lambda)$, and refer to $\lambda$ as the {\em scale}. Dwork et al.\ \cite{DMNS06} prove that the Laplace mechanism that the Laplace mechanism achieves $\e$-differential privacy, if it uses a noise scale $\lambda \ge GS(f)/\e$, where $GS(f)$ is the {\em global sensitivity} of $f$ defined as follows:
\begin{definition} [Global Sensitivity \cite{DMNS06}] \label{def:pre-sen}
Let $f$ be a function that maps a dataset $D$ into a vector of real numbers. The global sensitivity of $f$ is defined as
\begin{equation} \label{eqn:prelim-sen}
GS(f) = \max_{D,D'} \left|f(D) - f(D')\right|_1,
\end{equation}
where $D$ and $D'$ are any two neighboring datasets, and $|\cdot|_1$ denotes the $L_1$ norm.
\end{definition}
Intuitively, $GS(f)$ measures the maximum possible change in $f$'s output when we insert or remove one arbitrary tuple in $f$'s input. 

%A simple example for the Laplace mechanism and global sensitivity is to return the cardinality of the input, i.e., $f(D) = |D|$. As adding or deleting one tuple only changes the cardinality by one, it is easy to know that $GS(f) = 1$. Therefore, an $\e$-differentially private mechanism for releasing $f$ is to publish $|D|+\Lap(1/\e)$.

%Although there are many approaches to achieving differential privacy, the most fundamental one is the {\em Laplace mechanism}~\cite{DMNS06}.



%The Laplace mechanism releases the result of a function $f$
%that takes as input a dataset and outputs a numeric value.
%Given $f$, the Laplace mechanism transforms $f$ into a differentially
%private algorithm by adding i.i.d.\ noise (denoted as $\eta$) into
%the output value of $f$.
%The noise $\eta$ is sampled from a {\em Laplace distribution} $\operatorname{Lap}(\lambda)$ with the
%following pdf: $\Pr[\eta = x] = \frac{1}{2\lambda} e^{-|x|/\lambda}$.
%%The parameter $\lambda$ is proportional to the standard deviation of
%%$\eta$, and is referred to as the {\em scale} of the noise.}
%Dwork et al.\cite{DMNS06} prove that the Laplace mechanism achieves $\e$-differential privacy if $\lambda \ge GS(f)/\e$, where $GS(f)$ is the {\em global sensitivity} of $f$:
%%\begin{definition} [Global Sensitivity \cite{DMNS06}] \label{def:prelim-sen}
%%Let $f$ be a function that maps a graph into a fixed-size vector of real numbers. The {\em global sensitivity} of $f$ is defined as
%%\begin{equation} \label{eqn:prelim-sen}
%%GS^f = \max_{g, g'} \left\|f(g) - f(g')\right\|_1,
%%\end{equation}
%%where $\left\| \cdot \right\|_1$ denotes the $L_1$ norm, and $g$ and $g'$ are any two neighboring graphs.
%%\end{definition}
%\begin{definition} [Global Sensitivity \cite{DMNS06}] \label{def:pre-sen}
%Let $f$ be a function that maps a graph into a real number. The global sensitivity of $f$ is defined as
%\begin{equation} \label{eqn:prelim-sen}
%GS(f) = \max_{D,D'} \left|f(D) - f(D')\right|,
%\end{equation}
%where $D$ and $D'$ are any two neighboring datasets.
%\end{definition}
%Intuitively, $GS(f)$ measures the maximum possible change in $f$'s
%output when we add/delete one arbitrary tuple in $f$'s input.
%A simple example for the Laplace mechanism and global sensitivity is to return the cardinality of the input, i.e., $f(D) = |D|$. As adding or deleting one tuple only changes the cardinality by one, it is easy to know that $GS(f) = 1$. Therefore, an $\e$-differentially private mechanism for releasing $f$ is to publish $|D|+\Lap(1/\e)$.


\subsection{Spatial Decomposition}\label{sec:pre-spatial}
\begin{figure*}[t]
\centering
\includegraphics[height=26.5mm]{./2-Preliminaries/sd.pdf}\\
\vspace{-0mm}\caption{An example of spatial decomposition tree}
\label{fig:spatial}
\vspace{-0mm}
\end{figure*}

Spatial decompositions~\cite{S06book, D00book} are routinely used in managing spatial databases, with a long history stretching over decades. Formally, a spatial decomposition is a tree-structured decomposition of a geometric space into its sub-regions, along with the data points partitioned among leaves. As an example, Figure~\ref{fig:spatial} shows an instance of the best known decomposition model, namely, {\it quadtree}. Each node of the tree is associated with three members: the denotation, the corresponding region (marked in black) and the points located in it. The tree starts with a root node representing the entire space. Then nodes are recursively divided into four equal regions via horizontal and vertical lines through the midpoint of each dimension, until each leaf contains a small number of points (less than $5$ in this example). Note that leaves of the tree are disjoint regions whose union is exactly the entire space.

As in Figure~\ref{fig:spatial}, the spatial decomposition tree is skewed to fit the data, i.e., it grows deep into a dense area to build a fine model (e.g., $x_{13}$) while ignores the sparse parts (e.g., $x_{11}, x_{12}$ and $x_{14}$). Therefore, it is widely used as an efficient synopsis in modeling spatial data and answering a rich set of aggregate queries, particularly range-count queries. Specifically, given a count region $q$, e.g., the red dashed rectangle in Figure~\ref{fig:spatial}, we are interested to know how many points are located within $q$.
The counting algorithm starts from the root, then operates differently in the following three cases: (i) if the node does not intersect $q$, do nothing (e.g., $x_{11}$). (ii) if the node is fully contained in $q$, add the total number of associated points to the answer (e.g, $x_{24}$). (iii) if the node partially intersects $q$, recurse on its children if it is non-leaf (e.g., $x_0$ and $x_{13}$); otherwise, enumerate associated points and add the number of those in $q$ to the answer (e.g., $x_{14}$ and $x_{23}$). This algorithm is highly efficient as cases (i) and (ii) can significantly reduce the space of enumeration, especially when $q$ is small and large, respectively. In the next section, we will show how to build a differentially private spatial decomposition tree, and use it to answer range-count queries.



==> 4-Markov/Markov_-_backup.tex <==
\section{Markov Model}\label{sec:markov}

\begin{figure*}[t]
\centering
\hspace{-0mm}\includegraphics[height=21mm]{./4-Markov/mm.pdf}\\
\vspace{-0mm}\caption{An example of a prediction suffix tree}
\label{fig:markov}
\vspace{-0mm}
\end{figure*}

In this section, we present how to apply \tree to build private Markov models \cite{RST96, BEY04} for sequence data. Markov models are routinely used in modeling sequence data, with a long history stretching over decades. A Markov model is a stochastic model used to model randomly changing sequences where it is assumed that the future symbol depends only on its previous few symbols and not on the sequence that preceded them (that is, it assumes the Markov property \cite{RST96} of sequences). We make this combination of \tree and Markov model to address two drawbacks of previous solutions on private modeling of sequence data, e.g., prefix tree models \cite{CFDS12} and $n$-gram models \cite{CAC12}.
First, similar to the existing solutions for spatial decompositions \cite{CPSSY12}, they require a pre-defined limit $h$ on the height of the tree and the scale of noise injected to the model is proportional to $h$. As discussed in Sections~\ref{sec:intro} and \ref{sec:pre-spatial}, this design makes them hard to generate accurate models. Second, they rarely utilize the Markov property of sequence data to help build a better decomposition. For example, \cite{CAC12} decides if an $n$-gram should be expanded to $(n+1)$-grams, simply based on its noisy count. However, most Markov models also incorporate the {\em information gain of using a finer model} to decide if any further split is necessary. In particular, if further splitting a model gains little in terms of information, it should stop for the sake of conciseness. The extension of \tree to Markov models turns out to be significantly challenging, and we introduce a novel
approach that uses a surrogate function for the simple count
to build the model more accurately.

Let $D$ be a set of sequences over a finite alphabet $\I$, in which each sequence $s$ of length $|s|$ is an ordered list of symbols in $\I$, i.e., $s = x_1x_2\cdots x_{|s|}$, where $x_i\in \I$ for $i \in [1,|s|]$. To mark the start and end, we slightly modify the sequence by inserting the starting symbol $\$$ and the ending symbol $\&$ to its front and back, respectively. On the left side of Figure~\ref{fig:markov}, we present an example of sequence database over $\I = \left\{A, B\right\}$.
The literature on modeling such discrete sequences is rather extensive and offers various approaches to analyze and predict sequences over finite alphabet, among which prediction suffix trees are a well studied variant of variable length Markov models.
A prediction suffix tree (see the example in Figure~\ref{fig:markov}), over alphabet $\mathcal{I}$, is a tree of fanout $|\I|+1$ (symbols in $\I$ plus $\$$). Each node in the tree is associated with a {\em suffix} $s$ (denoted as ``dom'') and a {\em histogram of next symbol}, which predicts the next symbol when $s$ is the suffix of the current sequence. Note that all symbols in $D$ except $\$$'s contribute to the model, as each of them is the next symbol of a certain sequence. More specifically, each symbol $x_i \in \I\cup\left\{\&\right\}$ in sequence $\$x_1\cdots x_l$ is considered as the next symbol of the sequence ahead of it, i.e., $\$x_1\cdots x_{i-1}$, for $i\in[1,l]$.
The root of the tree $v_1$ corresponds to the entire space $\Omega$ of sequences, i.e., every sequence has an empty suffix. Therefore, its histogram contains all symbols in $D$ except $\$$'s. Then the suffix is recursively extended by one symbol {\em forward} each time, in order to split sequences into disjoint sub-domains. For example, $v_4$ represents all the sequences ending with $B$ and stores the next symbols of them, i.e., there are four occurrences of sequences ending with $B$, all of which are followed by $\&$.
The splitting process stops if any of the following criteria is met:
\begin{itemize}[itemsep=1pt, leftmargin=5mm]
\item $\dom(v)$ starts with $\$$, simply because that there is no more symbols before $\$$ (e.g., $v_2$ and $v_5$).

\item The sum of counts, referred to as {\em magnitude}, of the histogram is small. A small magnitude implies that $\dom(v)$ is rarely a suffix of sequences in the database, so there is no need to further split $v$ (e.g., $v_7$). This criterion has the similar intuition to the $n$-gram counts used in \cite{CAC12}.

\item The entropy of the histogram (when treated as a probability distribution) is small. This is an improvement over previous solutions. Node $v_4$ gives a good example of this case. The histogram of next symbol in $v_4$ has a zero entropy, which indicates that there is no uncertainty for the next symbol if the current sequence ends with symbol $B$. Therefore, the Markov property perfectly holds and splitting $v_4$ is just a waste.
\end{itemize}

Prediction suffix trees support a wide range of queries, among which the most important is to estimate {\em the occurrence of a sequence $s$}. Specifically, we initialize the query answer as the magnitude of the histogram in the root node. After that, for each symbol $x_i$ in $s$ $(1\le i \le |s|)$, we first find the node $v$ whose $\dom(v)$ is the longest suffix of sequence $x_1\cdots x_{i-1}$. Then multiply $ans$ with the probability of symbol $x_i$, derived from the next symbol histogram of $v$. By the end, we get the estimation.
Here we take the prediction suffix tree in Figure~\ref{fig:markov} and query sequence $s = AB$ as a working example. First, the query answer is set to the magnitude of the histogram in node $v_1$, i.e., $ans = 14$.
For the first symbol of sequence $x_1 = A$, we visit node $v_1$ as the empty is the only (of course longest) suffix of the empty. Then the answer is updated to $14 \cdot \frac{6}{14} = 6$. Note that this is actually the estimation for query $s = A$. Next we visit $v_3$ as it represents the longest suffix of $A$, and update $ans$ accordingly to $6\cdot \frac36 = 3$, which is the final estimation to be returned.
Moreover, the models also allow generating {\em synthetic sequence datasets}, but in a slightly different manner.
To generate one sequence, we (i) initiate a sequence with the starting symbol $s = \$$; (ii) find the leaf node $v$ whose $\dom(v)$ is a suffix of $s$, then sample the next symbol from its histogram; (iii) push the sampled symbol to the back of $s$; (iv) repeat (ii) and (iii) until the ending symbol $\&$ is sampled.

\subsection{Migrating to \tree}
To migrate the prediction suffix tree model to the framework of \tree, we need to make some modifications.
First of all, following the prior work \cite{CAC12}, our algorithm only considers the first $l_\top$ symbols (except $\$$) in each input sequence, in order to limit the impact of one tuple to the output. To explain, consider two neighboring datasets $D$ and $D'$, such that $D$ is obtained by inserting an {\em infinite} sequence $s$ into $D'$. Then $s$ will dominate the information in every node and invalid all analysis of differential privacy, if all its symbols are counted. However, with this length limit, it is easy to know that the impact of any sequence to the histogram of any node is bounded by $l_\top$, i.e., the sequence contributes at most $l_\top$ symbols to the histogram.

Second, the prediction suffix trees require three different criteria to decide whether a node should be split, while the spatial decompositions have only one. Among three criteria, the first one (i.e., whether $\dom(v)$ starts with $\$$) is easy to address as it is data-independent. We can solve it by changing the condition of splitting (Line 8 of Algorithm~\ref{alg:privtree}) to: {\bf if} $\dom(v)$ does not start with $\$$ {\bf and} $\hat{b}(v)>\theta$.

Third, since the latter two criteria are data-dependent, we need to design a new numeric function $c(\cdot)$ to incorporate both of them in making a split decision. As $c(\cdot)$ is no longer the tuple count used in spatial decompositions, here we generally refer to it as the score function of the node. The larger the score, the more likely the node is split. Let $h(v, i)$ be the count of symbol $i\in\I\cup\left\{\&\right\}$ in the histogram of node $v$, and $\mathrm{H}\left(h(v, \cdot)\right)$ be the entropy of that histogram.
The straightforward design of score function is to multiply the magnitude with the entropy of the histogram: $c(v) = \mathrm{H}\left(h(v, \cdot)\right) \cdot \sum_{i\in\I\cup\left\{\&\right\}}h(v,i).$ This function, although intuitive, could not serve as an legal score function due to the lack of monotonicity. For example, let $v$ be a tree node with a histogram $h(v, \cdot) = \left\{1,1\right\}$ and $u$ be the parent of $v$ with a histogram $h(u, \cdot) = \left\{2,1\right\}$. This score function gives $c(v) = 1\cdot2$ which is larger than $c(u) = 0.64\cdot 3$. As the correctness of Theorem~\ref{thm:alg:privacy} relies on the monotonicity of $c(\cdot)$, we have to redesign a new one, such that
\begin{enumerate}[itemsep=1pt, leftmargin=5mm]
\item $c(\cdot)$ is monotone, i.e., $c(v)\le c(u)$ if $u$ is an ancestor of $v$.

\item If the magnitude $\sum_{i\in\I\cup\left\{\&\right\}}h(v,i)$ or the entropy $\mathrm{H}\left(h(v, \cdot)\right)$ is small, $c(v)$ tends to be small.

%\item $c(\cdot)$ has a small sensitivity, with respect to its range.
\end{enumerate}

In what follows, we will clarify our construction of the score function. We notice that a histogram of small entropy always has a significant symbol $i$ whose count dominates others (see node $v_4$ of Figure~\ref{fig:markov}). This is reasonable as the small entropy implies the small uncertainty in the histogram, i.e., most symbols are $i$. To capture this property, we incorporate the idea of significant symbol to the score function, which is defined as
\begin{equation}
c(v) = \sum_{i\in\I\cup\left\{\&\right\}}h(v,i) - \max_{i\in\I\cup\left\{\&\right\}}h(v,i).
\end{equation}
The second half of r.h.s is the formal expression of the most significant count in the histogram. If the magnitude is small, then the score must be small no matter how large the most significant count is. On the other hand, if the entropy is small, then the most significant count that dominates the histogram will be very close to the magnitude, resulting in a small score as well. More importantly, we prove that this score function is a monotone function (Theorem~\ref{thm:newc:monotone}) of sensitivity $l_\top$ (Theorem~\ref{thm:newc:sens}).

\begin{theorem}\label{thm:newc:monotone}
$c(v)\le c(u)$ if $u$ is an ancestor of $v$ in the prediction suffix tree.
\end{theorem}
\begin{proof}
Since $u$ is an ancestor of $v$, all symbols in $v$' histogram also appear in $u$'s, making $h(v, i)
\le h(u, i)$ hold for every $i\in\I\cup\left\{\&\right\}$. Let $\max_v$ (resp. $\max_u$) be the most significant symbol in the histogram of $v$ (resp. $u$). We have
$c(v) = \sum_ih(v,i) - h(v,\max_v) \le
\sum_ih(v,i) - h(v,\max_u) \le \sum_ih(u,i) - h(u,\max_u) = c(u)$.
\end{proof}

\begin{theorem}\label{thm:newc:sens}
$S(c) = l_\top$.
\end{theorem}
\begin{proof}
It is easy to prove that modifying one symbol in the histogram changes the score by at most $1$. Let $D$ be the neighboring dataset of $D'$, obtained by inserting a sequence $s$ into $D'$. As we only consider the first $l_\top$ symbols of $s$ in the algorithm, the histogram will be modified by at most $l_\top$ symbols. Therefore, the change of the score is bounded by $l_\top$.
\end{proof}
With all these modifications listed above, we are able to apply \tree to build private prediction suffix trees for sequence datasets.

%From now on, we normalize the next symbol histogram of each node by $l$, such that the impact of one tuple to each node is bounded by $1$.


%\footnote{More generally, we could select $l$ privately by applying the exponential mechanism to return the $95$ quantile of sequence length in $D$ using a small fraction of privacy budget. For simplicity and brevity of the presentation, we manually select $l$ and assume it is public in this paper.}

Last, we summarize some tips about how to extend \tree to a general decomposition problem, Formally, we require that (i) $\dom(v) \subseteq \dom(u)$ if $u$ is an ancestor of $v$, vice versa; otherwise, $\dom(v) \cap \dom(u) = \emptyset$. (ii) $c(\cdot)$ is a function defined over $\dom(\cdot)$. In other words, any changes outside of $\dom(v)$ should not affect the value of $c(v)$. (iii) $c(\cdot)$ is a monotonic function of $\dom(\cdot)$, i.e., $c(v)\le c(u)$ if $\dom(v)\subseteq \dom(u)$. Clearly, the domain and score functions of spatial decompositions and predict suffix trees match these requirements.


